Deep image prior inpainting of ancient frescoes in the Mediterranean Alpine arc

The unprecedented success of image reconstruction approaches based on deep neural networks has revolutionised both the processing and the analysis paradigms in several applied disciplines. In the field of digital humanities, the task of digital reconstruction of ancient frescoes is particularly challenging due to the scarce amount of available training data caused by ageing, wear, tear and retouching over time. To overcome these difficulties, we consider the Deep Image Prior (DIP) inpainting approach which computes appropriate reconstructions by relying on the progressive updating of an untrained convolutional neural network so as to match the reliable piece of information in the image at hand while promoting regularisation elsewhere. In comparison with state-of-the-art approaches (based on variational/PDEs and patch-based methods), DIP-based inpainting reduces artefacts and better adapts to contextual/non-local information, thus providing a valuable and effective tool for art historians. As a case study, we apply such approach to reconstruct missing image contents in a dataset of highly damaged digital images of medieval paintings located into several chapels in the Mediterranean Alpine Arc and provide a detailed description on how visible and invisible (e.g., infrared) information can be integrated for identifying and reconstructing damaged image regions.

==> aa_DIPST.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection*{DIP with Style Transfer}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 Figure \ref{fig:dipst_architecture} = rete DIPST


% ***************************************************
\subsubsection{Enforcing style consistency via style transfer}  \label{ssec:st_dipst}

In this section, we discuss the basics of style transfer and we propose an application of style transfer for the inpainting of medieval frescoes. 
Style transfer is a neural technique introduced in 2015 \cite{https://doi.org/10.48550/arxiv.1508.06576}, with the general scope of defining a practical definition of style. The separation of content and style is achieved via the application of a pre-trained convoluted network and with the use of Gram matrices. This technique utilises a VGG-16 network \cite{https://doi.org/10.48550/arxiv.1409.1556}, which is used to compute two loss elements, the content and style loss respectively. The two losses are optimised to produce an image combining the style and content of two different images. 

When an image is passed through the pre-trained network, a filter activation from the last convoluted layer is obtained. This filter activation can be considered a source for a content match, and a loss term that enforces the feature response from the generated image to match the one obtained by the content source can thus be used.
A natural choice for the content loss is the quadratic loss of the feature response of the two images at the given layer $l$, called $F_1$ and $F_2$, where the layer $l$ is $ l\geq \bar{l} $ where $\bar{l}$ is a layer on the second half of the network. 

\begin{eqnarray}
L_{content}^l = \sum_{ij}{(F_1^{l_{ij}} - F_2^{l_{ij}})^2}
\end{eqnarray}

Unlike content, gathering style information requires a different mathematical formulation, as the simple match of a feature response would impose only a strict content match.
This problem is solved via the use of a correlation index between multiple feature responses, a task which is encoded by the use of Gram matrices. The Gram matrix is obtained by making the dot product of the feature response of a given layer by its transpose. A loss element can then be defined as a match between the Gram matrices of our style source and our newly created image, for different network layers. 
Mathematically a Gram matrix $G^l \in \mathbb{R}^{N_l \times N_l}$ where $G^{l}_{ij}$ is the inner product between the vectored feature map $i$ and $j$ in layer $l$ as reported in Equation \eqref{eq:gram_def}.

\begin{eqnarray}
G^{l} = F_{l} \odot F^{T}_{l}
\label{eq:gram_def}
\end{eqnarray}
The style loss can thus be defined as the quadratic loss of the difference between the two Gram matrices obtained with the original and the generated images, called respectively $G1$ and $G2$. 

\begin{eqnarray}
L_{style}^l = \sum_{ij}{(G_1^{l_{ij}} - G_2^{l_{jj}})^2}
\end{eqnarray}

By balancing the two loss elements, it is common to encounter artefacts and inconsistencies. This is usually solved by combining the loss terms with a form of regularisation, promoting local smoothness. For instance, one could consider the total variation (TV) loss. This subject is particularly relevant in the context of style transfer applied on videos, and some improvements were reached in the past years \cite{9204808}.

In the past years, additional research was conducted and brought significant improvements to style transfer \cite{8732370}. The major improvements include: the use of a generative transformation network for the creation of the image \cite{https://doi.org/10.48550/arxiv.1603.08155}, the computing of Gram Loss over horizontally and vertically translated features as proposed by Berger and Memisevic \cite{https://doi.org/10.48550/arxiv.1606.01286}, Li et al. made considerable contributions on the subject, proposing the demystification of style transfer \cite{https://doi.org/10.48550/arxiv.1701.01036}, showing that minimising Gram matrices between features is equivalent to minimising Maximum Mean Discrepancy (MMD) with second-order polynomial kernels, subtracting the mean of feature representations before computing Gram Loss, obtaining considerable improvements in eliminating discrepancy in scale \cite{https://doi.org/10.48550/arxiv.1703.01664}. 

\subsubsection*{Deep image prior style transfer}
\label{sec:dipst}

In this section we present a novel approach to inpainting, combining the deep image prior approach with style transfer elements. 
Our intent is to create an inpainting model with a methodology in-between the semantic approach of neural data-driven networks and the crafted prior algorithms. Also, the feasibility of finding a relevant dataset for a specific fresco is poor while the chance of finding a well-preserved coherent image from the same author is usually quite high. Therefore we approach the problem in such a way that we enable the leveraging of a single reference image for the inpainting process. Our experimental solution consists of a combined model, having the first part synthesising the inpainted image and the latter serving as a loss term enforcing compatibility with a style coherent image. 

The theoretical background of this novel architecture is to create a partially crafted prior, achieving the capability of semantic inpainting without the need for a large dataset of relevant images. Besides, the possibility of gathering information from a single relevant image is more correct for many applied tasks, such as restoration, where the restored piece should not be altered by information coming from undesired sources. With a data-driven method, this is particularly hard to enforce.


\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{images/dipst(2).png}
\caption{\label{fig:dipst_architecture} In this Figure we report the architecture of our DIPST model, showing a combination of deep image prior and a style transfer model}
\end{figure}



The general architecture of our model is reported in Figure \ref{fig:dipst_architecture}. Our approach consists in applying a two terms loss, including both the masked deep image prior loss and a style reference loss enforced via Gram matrices. The loss is reported in Equation \eqref{eq:dipst_loss} where we can observe the two parts, each being tuned via weight parameters $\alpha$ and $\beta$. The damaged image is represented as $I$, the inpainting mask as $m$ and $S$ is the style source image. The generative network $\Theta$ is dependent on the parameters $p$ with input noise $z$. In the left part of the loss we see the deep image prior contribution, in which we enforce the minimisation of the square difference between the generated image $\Theta_p(z)$ and the original image $I$. The mask is imposed via Hadamard's product with $m$. In the right part, we enforce the style coherence, which is obtained via the square difference between the Gram matrices $G$ obtained from the generated image $G_{\Theta_p(z)}$ and the reference image $G_S$. This operation is carried out for a selection of layers $l$.

\begin{eqnarray}
L_{inpaint} = \alpha|| (\Theta_p(z) - I)\odot m ||^2 + \beta \sum_l||G^l_{\Theta_p(z)} - G^l_S||^2
\label{eq:dipst_loss}   
\end{eqnarray}

The main intuition behind our practical implementation is to operate a match between the output tensor of the DIP hourglass network and the input tensor of the VGG-16 pre-trained model. Despite the complexity of the network structure, it is still a fully convolutional model, which means it can operate with multiple image sizes without restructuring the layers. 


\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{images/workflow_DIP_DIPST_dipst.png}
\caption{\label{fig:dipst} In this Figure we report ...}
\end{figure}


% ***************************************************
\subsubsection{Comparison DIP vs DIPST}

Figure \ref{fig:DIPST-DIP-fresco} and \ref{fig:DIPST_1}


\begin{figure}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaci.jpg}  
  \caption{square crop of a heavily damaged fresco}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaciMASK.png}  
  \caption{large mask applied on the image}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaci_style.jpg}  
  \caption{a preserved work by the same author}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.46\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaci_Sapiro.png}  
  \caption{Sapiro's algorithm}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.46\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaci_patch5.png}  
  \caption{patch inpainting}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.46\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaciDIP.png}  
  \caption{DIP}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.46\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/biazaciDIPST.png}  
  \caption{DIPST}
  \label{fig:sub-second}
\end{subfigure}
\caption{Comparison of inpainting methods dealing with a heavily damaged fresco. The paintings are from the chapel San Bernardino in Albenga, and the authors are Tommaso and Matteo Biazaci. In this case the picture is mostly missing with only a small portion preserved. The subject of the painting is hell, and it is part of a series by the same author. Luckily a coherent work by the same author is available, and it can be used a style reference for DIPST. 
}
\label{fig:DIPST-DIP-fresco}
\end{figure}

\begin{figure}[h!]
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/0100_1.jpg}  
  \caption{original image}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/0100_1mask&image.jpg}  
  \caption{inpainting mask}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/0100_2.jpg}  
  \caption{style source}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/DIP.png}  
  \caption{DIP}
  \label{fig:sub-second}
\end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
  \centering
  % include second image
  \includegraphics[width=\linewidth]{images/DIPST.png}  
  \caption{DIPST}
  \label{fig:sub-second}
\end{subfigure}
\caption{Using DISPT to achieve better inpainting results}
\label{fig:DIPST_1}
\end{figure}




